Design Space Exploration via Answer Set Programming Modulo Theories

The design of embedded systems, that are ubiquitously used in mobile devices and cars, is becoming continuously more complex such that efficient system-level design methods are becoming crucial. My research aims at developing systems that help the designer express the complex design problem in a declarative way and explore the design space to obtain divers sets of solutions with desirable properties. To that end, we employ knowledge representation and reasoning capabilities of ASP in combination with background theories. As a result, for the first time, we proposed a sophisticated methodology that allows for the direct integration of multi-objective optimization of non-linear objectives into ASP. This includes unique results of diverse sub-problems covered in several publications which I will present in this work.

==> img/architecture_tikz.tex <==
\definecolor{myblue}{HTML}{004A99}
\usetikzlibrary{intersections}
\begin{tikzpicture}
\tikzstyle{axis} = [-latex,thick]
\tikzstyle{axis2} = [-latex]
\tikzstyle{link} = [latex-latex, black]
\tikzstyle{mapping} = [-latex, black!60]
\tikzstyle{task} = [anchor=west,shape=rectangle,thick,text=white,minimum height=0.5cm, draw=black, fill=myblue, align=center, rounded corners=2,inner sep=0]
\tikzstyle{difftask} = [shape=circle,thick,text=white,minimum height=0.2cm, draw=black, fill=myblue, align=center,inner sep=0]
\tikzstyle{difftask2} = [shape=circle,thick,text=white,minimum height=0.1cm, draw=black, fill=myblue, align=center,inner sep=0]
\tikzstyle{router} = [icon,draw,fill=black!30!yellow,inner sep=0,minimum width=0.45cm,minimum height =0.3cm]
\tikzstyle{resource} = [rectangle,minimum width=0.3cm,minimum height=0.2cm,draw,fill=black!50!green,text=white]
\tikzstyle{route} = [->,black,line width=1.5]

\tikzstyle{textfield} = [draw,minimum height = 0.6cm,font=\footnotesize,text width=2cm,align=center]
\tikzstyle{decision} =[draw,diamond,text width=1.7cm,aspect=1.5,inner sep=0,align=center,font=\footnotesize,minimum width=2cm]


%\node [textfield,text width=] (v9) at (-1.4,-3.9) {Grounding};

%\draw [axis] (v4.west) --node[sloped,above=-3,font=\tiny]{depends on} (v3);

\coordinate (v5) at (-3.1,-3.1) {} {} {};
\coordinate (v6) at (-3.1,-8.8) {} {} {} {} {};
\coordinate (v7) at (0.3,-8.8) {} {} {} {} {} {};
\coordinate (v8) at (0.3,-3.1) {} {} {} {};
\draw[name path=API]  (v5) --coordinate[pos=0.5](v51)coordinate[pos=0.7](v52) (v6) -- (v7) -- (v8) -- cycle;
\node[anchor = north west,font=\small] at (v5) {Clingo};
\coordinate (s1) at (-2.8,-4.5) {} {} {} {} {} {} {};
\coordinate (s2) at (-2.8,-7.9) {} {} {} {} {} {} {} {};
\coordinate (s3) at (0,-7.9) {} {} {} {} {} {} {};
\coordinate (s4) at (0,-4.5) {} {} {} {} {} {};
\draw[] (s1) -- (s2) -- (s3) -- (s4) --node[midway] (smid){}  cycle;
\node [anchor=north west,font=\small] (s10) at (s1) {Binding};
%\draw[axis]  (v3) edge (v9);
%\draw[axis]  (v9) edge (smid.center);
\node [textfield,] (s9) at (-1.4,-5.7) {propagate and assign ASP decisions};



\coordinate (a1) at (0.5,-5.3) {} ;
\coordinate (a2) at (0.5,-8.8) {} {} {} {} {} ;
\coordinate (a3) at (6.2,-8.8) {} {} {} {} {} {} {} {} {} ;
\coordinate (a4) at (6.2,-5.3) {} {} {} {} {} {} {} ;
\draw  (a1) -- (a2) -- (a3) -- (a4) -- cycle;
\node[anchor = north west,font=\small] at (a1) {Optimization Propagator};
\node [textfield,minimum width=0cm,text width=,] (x3) at (1.9,-4.3) {evaluate\\objectives};

\coordinate (v1) at (-1.4,-4.9) {} {} {} {} {};
\coordinate (v2) at (-1.2,-4.9) {} {} {} {} {} {} {} {} {} {};
\coordinate (v4) at (0.8,-4.3) {} {} {} {} {} {} {} {} {};


\node [decision] (v10) at (4.4,-4.3) {};
\node[font=\footnotesize,text width=2cm,align=center,yshift=-1] at (v10) {constraints\\met?};
\draw[axis]  (x3) -- (v10);
\node [decision] (v11) at (4.4,-6.3) {};
\node[font=\footnotesize] at (v11) {dominated?};
\draw[axis]  (v10) --node[very near start, ,fill=white,font=\tiny,inner sep=1,outer sep=1]{yes}  (v11);
\node [decision] (v12) at (1.8,-6.3) {};
\node[font=\footnotesize,text width=2cm,minimum width=1,align=center,yshift=0.5] at (v12) {complete\\solution?};
\draw [axis] (v11) --node[pos=0.4, sloped,fill=white,font=\tiny,inner sep=1,outer sep=1]{no}  (v12);

\node [textfield,minimum width=0cm,text width=,fill=white] (v13) at (-1.4,-7.1) {restrict\\search space};
\draw [axis] (v13) edge (s9);
%\draw [axis] (v10) --node[midway, sloped,fill=white,font=\tiny,inner sep=0,outer sep=0]{conflict clause} (v13);
%\draw [axis] (v11) --node[midway, sloped,fill=white,font=\tiny,inner sep=0,outer sep=0]{conflict clause} (v13);
\coordinate (v40) at (0.4,-6.3) {} {} {} {} {} {} {} {};
\draw [axis] (v12) --node[midway, sloped,fill=white,font=\tiny,inner sep=1,outer sep=1]{no} (v40)|-(s9);



\coordinate (v17) at (3.9,-8.5);
\coordinate (v18) at (4.8,-8.5);
\coordinate (v16) at (3.9,-8.1);
\coordinate (v21) at (4.8,-8.1);
\coordinate (v22) at (5,-8.3);
\coordinate (v15) at (5,-7.9);
\coordinate (v14) at (4.1,-7.9);
\coordinate (v19) at (4.2,-8.3);
\coordinate (v20) at (4.5,-8.3);
\coordinate (v24) at (4.7,-7.9);
\coordinate (v25) at (4.7,-8.1);
\coordinate (v26) at (4.8,-7.8);
\coordinate (v27) at (4.1,-7.8);
\coordinate (v28) at (4,-8.1);
\coordinate (v29) at (4,-7.9);
\coordinate (v30) at (4.1,-8.1);
\coordinate (v31) at (4.9,-7.7);
\coordinate (v32) at (4.9,-8.1);
\coordinate (v33) at (4.2,-8.1);
\coordinate (v34) at (4.2,-7.7);
\draw[thick]  (v14) edge (v16);
\draw[thick]  (v14) edge (v15);
\draw[thick,fill=white]  (v16) -- (v17) -- (v18) -- (v22) -- (v15) -- (v14) -- cycle;
\draw [thick,fill=white] (v31) -- (v32)--(v33) --(v34) --cycle;
\draw[thick,fill=white] (v26)--(v27) -- (v30) -- (v21) -- cycle;
\draw [thick,fill=white] (v29) -- (v28)--(v25) --(v24) --cycle;
\draw [thick] (v15)--(v21) -- (v16);
\draw [thick,fill=white] (v18) -- (v21)--(v15);

%\draw[thick,fill=white]  (v16) -- (v17) -- (v18) -- (v22) -- (v15) -- (v14) -- cycle;
%\draw[thick,fill=white]  (v18) -- (v22) -- (v15) -- (v21) --cycle;
\draw [thick] (v19) -- (v20);
\coordinate (v38) at (1.8,-7.9) {} {} {} {} {} {} {} {} {} {};
\coordinate (v39) at (1.8,-8.7) {} {} {} {} {} {} {} {} {} {};
\draw [axis,-] (v12) --node[midway,fill=white,font=\tiny,pos=0.7,inner sep=1,outer sep=1,align=center]{yes} (v38) -- (v39);
\coordinate (v23) at (3.5,-7.2) {} {} {} {} {} {} {};
\coordinate (v37) at (5.3,-7.2) {} {} {} {} {} {} {};
\coordinate (v35) at (3.5,-8.6) {} {} {} {} {} {} {} {} {};
\coordinate (v36) at (5.3,-8.6) {} {} {} {} {} {} {};
\draw [] (v23) --node[midway](archleft){} (v35) --node[midway](archmid){} (v36) --node[midway](archright){} (v37) --node[midway](archtop){} cycle;
\node[anchor = north west,font=\footnotesize] at (v23) {Archive};



\draw [axis] (v38) --node[midway, sloped,fill=white,font=\tiny,inner sep=1,outer sep=1,align=center]{update} (archleft.center);% -- (archleft.center);
%\draw [axis] (v38) --node[midway, sloped,fill=white,font=\tiny,inner sep=0,outer sep=0]{conflict clause} (v13);

\draw[axis,open diamond-,dashed] (archtop.center)--node[midway, right=2,fill=white,font=\tiny,inner sep=1,outer sep=1,align=center]{check}(v11);%--node[midway, sloped,fill=white,font=\tiny,inner sep=0,outer sep=0,align=center]{check}(v11);
\coordinate (v41) at (6.1,-4.3) {} {} {};
\coordinate (v42) at (6.1,-6.3) {} {} {};
\coordinate (v45) at (6.1,-8.7) {} {} {} {} {};
\coordinate (v43) at (0.3,-8.7) {} {} {} {};
\coordinate (v44) at (-1.4,-8.7) {} {} {};
\draw [axis](v10) --node[fill=white,font=\tiny]{no} (v41) -- (v42)--(v45) -- (v43) --node[midway,, sloped,fill=white,font=\tiny,inner sep=0,outer sep=0]{conflict clauses} (v44) -- (v13);
\draw [axis,-] (v11) --node[midway,sloped,pos=0.5,font=\tiny,fill=white,inner sep=1,outer sep=1]{yes} (v42);
%\draw [thick] (v38) edge (v44);
\coordinate (v47) at (0.5,-5.1) {};
\coordinate (v48) at (6.2,-5.1) {} {};
\coordinate (v49) at (6.2,-3.1) {} {} {};
\coordinate (v46) at (0.5,-3.1) {} {};
\draw (v46) -- (v47) -- (v48) -- (v49) -- cycle;
\node[anchor = north west,font=\small] at (v46) {Theory Propagator};
%\draw [axis] (v80) -- (v9);
\draw[axis]  (s9) |-node[pos=0.7,sloped,font=\tiny,fill=white,inner sep=1,outer sep=1]{(partial) assignment} (x3);
\draw (-7.3,-3.1) -- (-4.3,-3.1) --coordinate[midway](v101) (-4.3,-5.4)  -- (-7.3,-5.4) -- cycle;
\draw (-7.3,-5.6) -- (-7.3,-8.8) -- (-4.3,-8.8) --coordinate[midway](v100) (-4.3,-5.6) -- cycle;
\node [difftask] (v50) at (-6.8,-6.6) {};


\node [difftask] (v54) at (-6,-6.8) {};
\node [difftask] (v53) at (-6.3,-6.4) {};

\node [difftask] (v59) at (-5.8,-6.4) {};
\node [difftask] (v61) at (-4.9,-6.6) {};
\node [difftask] (v60) at (-5.4,-6.6) {};


%\draw [axis2] (v58) edge (v50);

\node [resource] (v63) at (-6.6,-7.9) {};
\node [resource] (v65) at (-5.9,-7.9) {};
\node [resource] (v68) at (-6.6,-8.5) {};
\node [resource] (v69) at (-5.9,-8.5) {};
\node [resource] (v67) at (-5.2,-7.9) {};
\node [resource] (v70) at (-5.2,-8.5) {};
\node [resource] (v62) at (-6.6,-7.3) {};
\node [resource] (v64) at (-5.9,-7.3) {};
\node [resource] (v66) at (-5.2,-7.3) {};
\draw [link] (v62) edge (v63);
\draw [link] (v62) edge (v64);
\draw [link] (v63) edge (v65);
\draw [link] (v64) edge (v66);
\draw [link] (v66) edge (v67);
\draw [link] (v67) edge (v65);
\draw [link] (v63) edge (v68);
\draw [link] (v68) edge (v69);
\draw [link] (v69) edge (v70);
\draw [link] (v65) edge (v69);
\draw [link] (v67) edge (v70);
\draw [link] (v64) edge (v65);

\draw [axis2] (v50) edge (v53);
\draw [axis2] (v50) edge (v54);
\draw [axis2] (v53) edge (v59);
\draw [axis2] (v54) edge (v60);
\draw [axis2] (v59) edge (v60);
\draw [axis2] (v60) edge (v61);
\draw [axis2] (v53) edge (v54);
\draw [mapping] (v50) edge (v68);
\draw [mapping] (v53) edge (v64);
\draw [mapping] (v54) edge (v62);
\draw [mapping] (v59) edge (v66);
\draw [mapping] (v60) edge (v65);
\draw [mapping] (v61) edge (v67);
\draw [mapping] (v54) edge (v70);
\draw [mapping] (v59) edge (v69);
\draw [mapping] (v50) edge (v65);
\draw [mapping] (v60) edge (v63);
\draw [mapping] (v61) edge (v66);
\node[anchor=north west,font=\small] at (-7.3,-3.1) {Problem Definition};
\node[anchor=north west,font=\small] at (-7.3,-5.6) {Problem Instance};
\node[anchor=north west,font=\scriptsize,text=gray] at (-7.1,-3.7) {rule1(X,R):-fact1(X,R).};
\node[anchor=north west,font=\scriptsize,text=gray] at (-7.1,-4.1) {rule2(X):-fact2(X).};
\node[anchor=north west,font=\scriptsize,text=gray] at (-7.1,-4.5) {:-fact1(X,R),fact1(Y,R).};

\path[name path=tmp1] (v100) -- +(2,0);
\path[name intersections={of=API and tmp1,by={INT}}];
%\draw[axis] (v100) --node[midway,fill=white,font=\tiny,inner sep=0]{grounded} (INT);
\path[name path=tmp2] (v101) -- +(2,0);
\path[name intersections={of=API and tmp2,by={INT2}}];
%\draw[axis] (v101) --node[midway,fill=white,inner sep=0,font=\tiny]{grounded} (INT2);

\draw[axis] (v101) -- +(0.3,0) |- (v51);
\draw[axis] (v100) -- +(0.3,0) |-node[pos=0.55,anchor=west,font=\tiny,fill=white,inner sep=0,outer sep=0]{ground} (v51);

%\draw[axis,-] (v100) -| (mid.west); 

\draw[axis,latex-latex] (6.9,-5.5) node[left, font=\tiny] (v75) {} --node[midway,font=\tiny,rotate=90,above=-2]{objective 2} (6.9,-8.3) 
-- node[midway,font=\tiny,below=-2]{objective 1}
(9.5,-8.3) 
node[font=\tiny,below=2] (v76) {};
\node [difftask2] (v3) at (7.1,-5.8) {};
\node [difftask2] (v9) at (7.3,-6.5) {};
\node [difftask2] (v52) at (7.6,-7.3) {};
\node [difftask2] (v55) at (8,-7.6) {};
\node [difftask2] (v56) at (8.4,-8) {};
\node [difftask2] (v57) at (9.2,-8.2) {};
\node [difftask2] (v58) at (7.3,-6.2) {};
\node [difftask2] (v74) at (8.7,-8.1) {};
\node [difftask2] (v71) at (7.4,-7) {};
\node [difftask2] (v72) at (7.8,-7.5) {};
\node [difftask2] (v73) at (8.2,-7.9) {};
\draw (v3) -- (v58) -- (v9) -- (v71) -- (v52) -- (v72) -- (v55) -- (v73) -- (v56) -- (v74) -- (v57);
\draw[densely dotted,gray] (v37) -- (v75);
\draw[densely dotted,gray] (v36) -- (v76);
\node[font=\small,align=center] at (8.5,-6.5) {Objective\\Space};
\end{tikzpicture}

==> img/overview.tex <==
\definecolor{myblue}{HTML}{004A99}

\begin{tikzpicture}[]

\tikzstyle{input} = [anchor=west,shape=rectangle,thick,text=white,minimum width=2cm, draw=black, fill=myblue, align=center, rounded corners=2,inner sep=4]
\tikzstyle{task} = [rectangle,minimum width=2cm,minimum height=0.3cm,draw,fill=black!50!green,text=white,align=center,anchor = west,inner sep=4]
\tikzstyle{output} = [rectangle,minimum width=2cm,minimum height=0.3cm,draw,fill=orange,text=white,align=center,anchor = west,inner sep=4]
\tikzstyle{arrow} = [-latex,very thick]
\tikzstyle{noarrow} = [draw, black, -,thick]
\tikzstyle{resource} = [thick, minimum width=0.4cm, minimum height=0.4cm,fill=gray,draw=black]


\draw[thick, draw,fill=myblue,fill opacity=0.3]  (-4.3,1.3) rectangle (1.1,-1.8) node (v12) {};
\draw[thick, draw,fill=myblue,fill opacity=0.3]  (6.8,1.3) rectangle (12.7,-1.8);
\fill[thick,draw,fill=myblue,fill opacity=0.3]  (-4.5,1.5) rectangle (12.9,-2);
\node[anchor=south] at (-1.6,-1.8) {Topic \textbf{A}};
\node[anchor=south] at (9.75,-1.8) {Topic \textbf{B}};
\node[anchor=south] at (4.2,-2) {Topic \textbf{C}};

%\draw[fill=white]  (-4.1,1.2) -- (-4.1,-1.2) -- node[midway,above,fill=white]{Design Time Decisions} (6.4,-1.2) -- (6.4,1.2) --cycle ;
\draw[fill=white]  (-4.1,1.2) -- (-4.1,-1.2) -- node[midway,above=-2] (midpoint){} (6.4,-1.2) -- (6.4,1.2) --cycle ;
\draw[thick] (1.1,1.3) -- (v12);
\node[fill=white,anchor=south] at (midpoint) {Design Time Decisions};


\node[task] (v1) at (-4,0) {Automated\\Platform \\Generation};

\node [task] (v2) at (-1.25,0) {Feasibility\\Filter};
\node [task] (v3) at (1.5,0) {Pareto\\Filter};
\draw [arrow] (v1) -- (v2);
\draw [arrow] (v2) -- (v3);
\node [output] (v4) at (4.25,0) {Optimized \\Computing \\Platforms};

\draw [arrow,latex-] (v1.135) -- ++(0,1.5);

\node [input] (v7) at (-1.5,2.1) {Resource\\Database};
\node [input,dashed,fill=myblue!80] (v71) at (1,2.1) {Expert \\Guidance};
\node [input] (v6) at (-4,2.1) {Typical \\Workload};
\node[input] (v5) at (3.5,2.1) {Quality\\Criteria};


% \draw [noarrow] (5,1.4) rectangle (7.4,-1);
% \draw [noarrow] (5,-1.4) rectangle (7.4,-3);
% 
% \node [resource,fill=gray!70] (v4) at (5.4,1) {};
% \node [resource,fill=gray] (v5) at (6.2,1) {};
% \node [resource,fill=gray!70] (v10) at (7,1) {};
% \node [resource,fill=gray!70] (v6) at (5.4,0.2) {};
% \node [resource,fill=gray!70] (v9) at (6.2,0.2) {};
% \node [resource,fill=gray!70] (v11) at (7,0.2) {};
% \node [resource] (v7) at (5.4,-0.6) {};
% \node [resource] (v8) at (6.2,-0.6) {};
% \node [resource] (v12) at (7,-0.6) {};
% 
% \draw [noarrow] (v4) edge (v5);
% \draw [noarrow] (v4) edge (v6);
% \draw [noarrow] (v6) edge (v7);
% \draw [noarrow] (v7) edge (v8);
% \draw [noarrow] (v8) edge (v9);
% \draw [noarrow] (v9) edge (v6);
% \draw [noarrow] (v5) edge (v9);
% \draw [noarrow] (v10) edge (v5);
% \draw [noarrow] (v11) edge (v9);
% \draw [noarrow] (v11) edge (v12);
% \draw [noarrow] (v12) edge (v8);
% \draw [noarrow] (v11) edge (v10);
% 
% 
% \node [resource] (v13) at (5.4,-2) {};
% \node [resource,fill=gray!70] (v15) at (6.2,-2) {};
% \node [resource] (v17) at (7,-2) {};
% \coordinate (v14) at (5.4,-2.6) {} {};
% \coordinate (v16) at (6.2,-2.6) {} {};
% \coordinate (v18) at (7,-2.6) {} {};
% 
% \draw[noarrow]  (v13) -- (v14) -- (v16)--(v15);
% \draw[noarrow] (v15)--(v16)--(v18)--(v17);

%\draw[fill=white]  (7,1.2) -- (7,-1.2) -- node[midway,above]{Run Time Decisions\phantom{g}\hspace*{-0.5em}} (12.5,-1.2) -- (12.5,1.2) --cycle ;
\draw[fill=white]  (7,1.2) -- (7,-1.2) -- node[midway,above=-2] (midpoint){} (12.5,-1.2) -- (12.5,1.2) --cycle ;
\node[fill=white,anchor=south] at (midpoint) {Run Time Decisions\phantom{g}\hspace*{-0.5em}};
\draw [arrow] (v3) -- (v4);
\draw [arrow] (v5.south) -- ++(0,-0.5) node{} -|  (v3.north);
%\draw [arrow] (v6.225) -- ++(0,-0.5) node{} -| (v1.135);
\draw [arrow] (v7.south) -- ++(0,-0.5) node{} -|  (v1);


\node [task] (v9) at (7.1,0) {Embedded\\Mapper};
\node [output] (v11) at (9.7,0) {Updated\\Implementation};
\node [input] (v10) at (9.4,2.1) {Current \\Implementation};
\node [input] (v8) at (7.1,2.1) {New\\Application};
\draw [arrow] (v8.south) -- ++(0,-0.5) node{} -| (v9.135);
\draw [arrow] (v10.south) -- ++(0,-0.5) node{} -|  (v9.45);
\draw [arrow,dashed,double] (v4) -- (v9);
\draw [arrow] (v9) -- (v11);
\draw [arrow,-open diamond,dashed] (v11.0) -- ++(0.2,0.0) node{} |- (v10.0);
\draw [arrow,dashed] (v71.south) -- ++(0,-0.6) node{} -|  (v1.45);




\end{tikzpicture}
